Images in Language Space: Exploring the Suitability of Large Language Models for Vision & Language Tasks

Large language models have demonstrated robust performance on various language tasks using zero-shot or few-shot learning paradigms. While being actively researched, multimodal models that can additionally handle images as input have yet to catch up in size and generality with language-only models. In this work, we ask whether language-only models can be utilised for tasks that require visual input -- but also, as we argue, often require a strong reasoning component. Similar to some recent related work, we make visual information accessible to the language model using separate verbalisation models. Specifically, we investigate the performance of open-source, open-access language models against GPT-3 on five vision-language tasks when given textually-encoded visual information. Our results suggest that language models are effective for solving vision-language tasks even with limited samples. This approach also enhances the interpretability of a model's output by providing a means of tracing the output back through the verbalised image content.

==> ACL 2023 - Vision-Language Tasks with LLMs/tables/table1.tex <==
\begin{table*}[!ht]
\centering
\small

\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multicolumn{2}{|c|}{\textbf{}}                                    & \multicolumn{5}{c|}{\textbf{Datasets}}                                                                                                                                                                                                                                        \\ 
\hline
\textbf{LLM}      & \textbf{Run}                                   & \begin{tabular}[c]{@{}c@{}}MAMI\\(F1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}MVSA\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HF\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}NLVR2\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}OK-VQA\\ (Acc)\end{tabular}  \\ 
\hline
%%% FLAN-T5
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Flan-T5}}} & adaptive, n=2                 & 64.4                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                 & -                                                  & 35.2                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                 & -                                                  & -                                                   & 57.4                                              & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & -                                                 & 31.7                                                 & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                   & -                                                  & -                                                   & -                                                 & -                                                    & \textbf{35.4}                                                       \\ 
\hline
%                   & static, C, T, blip, n=2, k=1                   & -                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
% \hline
%%% GPT-3 
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{GPT-3}}} & adaptive, n=2                 & \textbf{69.2}                                               & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                 & -                                                  & 64.3                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & \textbf{58.8}                                              & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & -                                                 & \textbf{63.0}                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                  & -                                                  & -                                                   & -                                                 & -                                                    & 25.9                                                       \\ 
\hline
                  


%%% OPT
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{OPT}}} & adaptive, n=3                 & 22.4                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=3                 & -                                                  & 14.4                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=1                   & -                                                  & -                                                   & 44.4                                                & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=1                   & -                                                  & -                                                   & -                                                 & 47.7                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=1                   & -                                                  & -                                                   & -                                                 & -                                                    & 10.0                                                       \\ 
\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{T0pp}}} & adaptive, n=1                 & 46.0                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=0                 & -                                                  & \textbf{68.1}                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=1                   & -                                                  & -                                                   & 53.6                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=0                  & -                                                  & -                                                   & -                                                 & 58.6                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                   & -                                                  & -                                                   & -                                                 & -                                                    & 20.3                                                       \\ 
\hline

\multicolumn{2}{|c|}{\textbf{Fine-tuned Vision-Language Models}}   & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{2}{|l|}{\citet{zhang-wang-2022-srcb} }                        & 83.4                                               & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/mir/CheemaHME21}}                    & -                                                  & 75.3                                                & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/nips/KielaFMGSRT20}}                 & -                                                  & -                                                   & 66.1                                              & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/eccv/ChenLYK0G0020}}                 & -                                                  & -                                                   & -                                                 & 79.5                                                 & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/aaai/WuLSM22}}                       & -                                                  & -                                                   & -                                                 & -                                                    & 41.4                                                    \\ 
\hline
\multicolumn{2}{|l|}{\citet{schwartz-2021-ensemble} }                      & -                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|c|}{\textbf{Few-shot Models}}                     & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/aaai/YangGW0L0W22} }                 & -                                                  & -                                                   & -                                                 & -                                                    & 48.0                                                    \\ 
\hline
\multicolumn{2}{|l|}{\citet{gui-etal-2022-kat}}                            & -                                                  & -                                                   & -                                                 & -                                                    & 54.4                                                    \\
\hline
\end{tabular}
\caption{The results for all evaluated datasets including the results of the models that are fine-tuned on vision-language datasets. We include the best scoring configuration for each language model and the dataset. \textit{adaptive}: it indicates the selection of in-context samples as described in Section~\ref{subsec:sample_selection}, and \textit{n} indicates the number of selected samples in prompts. All runs use \textit{BLIP} image captions as image-as-text representation.}
\label{tab:table1}
\end{table*}

==> ACL 2023 - Vision-Language Tasks with LLMs/tables/table2.tex <==

\begin{table*}[ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{LLM}} & \multicolumn{1}{c|}{\textbf{Image-Text}} & \multicolumn{1}{c|}{\textbf{n=0}} & \multicolumn{1}{c|}{\textbf{n=1}} & \multicolumn{1}{c|}{\textbf{n=2}} & \multicolumn{1}{c|}{\textbf{n=3}} & \multicolumn{1}{c|}{\textbf{n=6}} & \multicolumn{1}{c|}{\textbf{n=12}} & \multicolumn{1}{c|}{\textbf{T}} & \multicolumn{1}{c|}{\textbf{S}} \\ \hline

% MAMI
\multirow{3}{*}{MAMI}   & Flan-T5  & ofa   &     &    &    &    &   &   &   & static   \\ \cline{2-11} 
 & Flan   & blip   &    &     &    &      &     &    &   & adaptive \\ \cline{2-11} 
  & Flan   & blip   &    &     &    &      &     &    &   & adaptive \\ \hline

% MVSA

% HF
\multirow{3}{*}{HF}   & Flan-T5  & blip   &  55.2   &  57.4  &    &  56.0  & 57.4  & 57.0  &  \checkmark & adaptive   \\ \cline{2-11} 

& Flan-T5  & blip   &  55.2   &  57.4  &    &  56.0  & 57.4  & 57.0  &  \xmark & adaptive   \\ \cline{2-11}

  & Flan-T5   & blip   &    &     &    &      &     &    &   & adaptive \\ \hline

% NLVR2

% OK-VQA

% VD
\end{tabular}
\caption{The results for all evaluated datasets including the results for the baseline models. We include the best scoring configuration for each language model and the dataset. \textbf{C}: caption, \textbf{V}: visual tags, \textbf{T}: task description,  \textbf{n}: the number of in-context samples in a prompt, \textbf{k}: the number of times the same evaluation sample is prompted with different in-context samples, \textbf{ofa}: image caption generated by the model OFA (One for all), \textbf{blip}: image caption generated by the model BLIP, \textbf{static}: selecting random n in-context samples, \textbf{adaptive}: selection of the most similar n samples based on the similarity between evaluation and training samples.}
\label{tab:table2}
\end{center}
\end{table*}

==> tables/table1.tex <==
\begin{table*}[!ht]
\centering
\small

\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multicolumn{2}{|c|}{\textbf{}}                                    & \multicolumn{5}{c|}{\textbf{Datasets}}                                                                                                                                                                                                                                        \\ 
\hline
\textbf{LLM}      & \textbf{Run}                                   & \begin{tabular}[c]{@{}c@{}}MAMI\\(F1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}MVSA\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HF\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}NLVR2\\(Acc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}OK-VQA\\ (Acc)\end{tabular}  \\ 
\hline
%%% FLAN-T5
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Flan-T5}}} & adaptive, n=2                 & 64.4                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                 & -                                                  & 35.2                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                 & -                                                  & -                                                   & 57.4                                              & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & -                                                 & 31.7                                                 & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                   & -                                                  & -                                                   & -                                                 & -                                                    & \textbf{35.4}                                                       \\ 
\hline
%                   & static, C, T, blip, n=2, k=1                   & -                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
% \hline
%%% GPT-3 
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{GPT-3}}} & adaptive, n=2                 & \textbf{69.2}                                               & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                 & -                                                  & 64.3                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & \textbf{58.8}                                              & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                   & -                                                  & -                                                   & -                                                 & \textbf{63.0}                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=2                  & -                                                  & -                                                   & -                                                 & -                                                    & 25.9                                                       \\ 
\hline
                  


%%% OPT
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{OPT}}} & adaptive, n=3                 & 22.4                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=3                 & -                                                  & 14.4                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=1                   & -                                                  & -                                                   & 44.4                                                & -                                                    & -                                                       \\ 
\cline{2-7}
                  & static, n=1                   & -                                                  & -                                                   & -                                                 & 47.7                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=1                   & -                                                  & -                                                   & -                                                 & -                                                    & 10.0                                                       \\ 
\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{T0pp}}} & adaptive, n=1                 & 46.0                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=0                 & -                                                  & \textbf{68.1}                                                   & -                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=1                   & -                                                  & -                                                   & 53.6                                                 & -                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=0                  & -                                                  & -                                                   & -                                                 & 58.6                                                    & -                                                       \\ 
\cline{2-7}
                  & adaptive, n=3                   & -                                                  & -                                                   & -                                                 & -                                                    & 20.3                                                       \\ 
\hline

\multicolumn{2}{|c|}{\textbf{Fine-tuned Vision-Language Models}}   & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{2}{|l|}{\citet{zhang-wang-2022-srcb} }                        & 83.4                                               & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/mir/CheemaHME21}}                    & -                                                  & 75.3                                                & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/nips/KielaFMGSRT20}}                 & -                                                  & -                                                   & 66.1                                              & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/eccv/ChenLYK0G0020}}                 & -                                                  & -                                                   & -                                                 & 79.5                                                 & -                                                       \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/aaai/WuLSM22}}                       & -                                                  & -                                                   & -                                                 & -                                                    & 41.4                                                    \\ 
\hline
\multicolumn{2}{|l|}{\citet{schwartz-2021-ensemble} }                      & -                                                  & -                                                   & -                                                 & -                                                    & -                                                       \\ 
\hline
\multicolumn{2}{|c|}{\textbf{Few-shot Models}}                     & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{2}{|l|}{\citet{DBLP:conf/aaai/YangGW0L0W22} }                 & -                                                  & -                                                   & -                                                 & -                                                    & 48.0                                                    \\ 
\hline
\multicolumn{2}{|l|}{\citet{gui-etal-2022-kat}}                            & -                                                  & -                                                   & -                                                 & -                                                    & 54.4                                                    \\
\hline
\end{tabular}
\caption{The results for all evaluated datasets including the results of the models that are fine-tuned on vision-language datasets. We include the best scoring configuration for each language model and the dataset. \textit{adaptive}: it indicates the selection of in-context samples as described in Section~\ref{subsec:sample_selection}, and \textit{n} indicates the number of selected samples in prompts. All runs use \textit{BLIP} image captions as image-as-text representation.}
\label{tab:table1}
\end{table*}

==> tables/table2.tex <==

\begin{table*}[ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{LLM}} & \multicolumn{1}{c|}{\textbf{Image-Text}} & \multicolumn{1}{c|}{\textbf{n=0}} & \multicolumn{1}{c|}{\textbf{n=1}} & \multicolumn{1}{c|}{\textbf{n=2}} & \multicolumn{1}{c|}{\textbf{n=3}} & \multicolumn{1}{c|}{\textbf{n=6}} & \multicolumn{1}{c|}{\textbf{n=12}} & \multicolumn{1}{c|}{\textbf{T}} & \multicolumn{1}{c|}{\textbf{S}} \\ \hline

% MAMI
\multirow{3}{*}{MAMI}   & Flan-T5  & ofa   &     &    &    &    &   &   &   & static   \\ \cline{2-11} 
 & Flan   & blip   &    &     &    &      &     &    &   & adaptive \\ \cline{2-11} 
  & Flan   & blip   &    &     &    &      &     &    &   & adaptive \\ \hline

% MVSA

% HF
\multirow{3}{*}{HF}   & Flan-T5  & blip   &  55.2   &  57.4  &    &  56.0  & 57.4  & 57.0  &  \checkmark & adaptive   \\ \cline{2-11} 

& Flan-T5  & blip   &  55.2   &  57.4  &    &  56.0  & 57.4  & 57.0  &  \xmark & adaptive   \\ \cline{2-11}

  & Flan-T5   & blip   &    &     &    &      &     &    &   & adaptive \\ \hline

% NLVR2

% OK-VQA

% VD
\end{tabular}
\caption{The results for all evaluated datasets including the results for the baseline models. We include the best scoring configuration for each language model and the dataset. \textbf{C}: caption, \textbf{V}: visual tags, \textbf{T}: task description,  \textbf{n}: the number of in-context samples in a prompt, \textbf{k}: the number of times the same evaluation sample is prompted with different in-context samples, \textbf{ofa}: image caption generated by the model OFA (One for all), \textbf{blip}: image caption generated by the model BLIP, \textbf{static}: selecting random n in-context samples, \textbf{adaptive}: selection of the most similar n samples based on the similarity between evaluation and training samples.}
\label{tab:table2}
\end{center}
\end{table*}
